VMap: An Interactive Rectangular Space-filling Visualization for Map-like Vertex-centric Graph Exploration

We present VMap, a map-like rectangular space-filling visualization, to perform vertex-centric graph exploration. Existing visualizations have limited support for quality optimization among rectangular aspect ratios, vertex-edge intersection, and data encoding accuracy. To tackle this problem, VMap integrates three novel components: (1) a desired-aspect-ratio (DAR) rectangular partitioning algorithm, (2) a two-stage rectangle adjustment algorithm, and (3) a simulated annealing based heuristic optimizer. First, to generate a rectangular space-filling layout of an input graph, we subdivide the 2D embedding of the graph into rectangles with optimization of rectangles' aspect ratios toward a desired aspect ratio. Second, to route graph edges between rectangles without vertex-edge occlusion, we devise a two-stage algorithm to adjust a rectangular layout to insert border space between rectangles. Third, to produce and arrange rectangles by considering multiple visual criteria, we design a simulated annealing based heuristic optimization to adjust vertices' 2D embedding to support trade-offs among aspect ratio quality and the encoding accuracy of vertices' weights and adjacency. We evaluated the effectiveness of VMap on both synthetic and application datasets. The resulting rectangular layout has better aspect ratio quality on synthetic data compared with the existing method for the rectangular partitioning of 2D points. On three real-world datasets, VMap achieved better encoding accuracy and attained faster generation speed compared with existing methods on graphs' rectangular layout generation. We further illustrate the usefulness of VMap for vertex-centric graph exploration through three case studies on visualizing social networks, representing academic communities, and displaying geographic information.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> old_5_graph_embedding.tex <==
\subsection{Graph Embedding}

The graph (or, network) embedding serves the basis of VMap layouts. We first embed vertices of a graph into a high-dimensional latent space and perform clustering on the high-dimensional space to approximate communities of vertices. Second, we embed vertices into a two-dimensional latent space and perform rectangular subdivision on the 2D space. After the graph embedding, each vertex is assigned a high-dimensional latent vector in the high-dimensional space and a 2D latent vector in the 2D space. 

% % \setlength{\belowcaptionskip}{-10pt}
% \begin{figure}[htb]
%   \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
%   \includegraphics[width=0.8\columnwidth]{les-miserables-graph}
%   % \vspace{-1em}
%   \caption{We show the co-occurrence network of characters in a novel \textit{Les Mis\'{e}rables} \cite{hugo1887miserables}, which is illustrated in Sect.~\ref{sect:app_les} with details. The graph drawing result is produced by a combined method of node2vec and t-SNE. Each circle represents a character. The radius of a given circle encodes the total number of co-occurence for the corresponding character with other characters; higher co-occurence numbers of the character indicates that the character is active in the novel. Co-occurred characters are connected by links. Colors encode communities of characters, and are suggested by ColorBrewer \cite{brewer2019colorbrewer}. }
%   % \vspace{-1.5em}
%   \label{fig:les-miserables-graph}
% \end{figure}
% % \setlength{\belowcaptionskip}{0pt}


\subsubsection{High-dimensional Embedding and Clustering of Vertices}

% The above three constraints have no contradiction and are consistent under the principle of \textit{homophily} \cite{mcpherson2001birds}, which is the primary force to form the social networks \cite{yang2014overlapping}. \textit{Homophily} \cite{mcpherson2001birds} is the principle in sociology that a connection between similar individuals happens at a higher rate than among dissimilar individuals. If we consider that similar individuals form communities (e.g., various academic communities formed by similar interests), hence, we can observe a feature that individuals have high densities of edges within communities (i.e., more intra-community edges) and low concentrations between communities (i.e., fewer inter-community edges) in real networks \cite{fortunato2010community}. 

To embed graphs into a high-dimensional space, \textit{node2vec} \cite{grover2016node2vec} proposed by Grover and Leskovec shows its power to capture different kinds of graph structures. The parameter $q$ of node2vec controls which graph structures to capture. To embed connected vertices closely and capture global communities of a given graph, $q$ should be smaller than one and is set to $0.5$ in our paper by the guidance of the node2vec paper \cite{grover2016node2vec}. The communities of vertices are important to understand graph structures \cite{fortunato2010community} hence are valuable to be displayed by the visual representations. We estimate communities of vertices by performing clustering of vertices on the high-dimensional latent space. Suggested by the node2vec paper \cite{grover2016node2vec}, we choose the \textit{k-means} method to perform clustering on the vertices in the latent space. 

% If the data contain the community or cluster information, we directly use the information for the next layout methods. Otherwise, individuals that are highly interconnected are more likely to belong to the same community \cite{grover2016node2vec}; hence, 

After obtaining the communities of vertices, we create a two-level hierarchical graph, in which the top layer describes connections between communities, and the bottom layer records relations of vertices. The top-layer graph of communities, called \textit{community graph} hereafter, is also a vertex-weighted graph. Weights of communities are the weight sum of the vertices in the communities. The edges between every two communities are the aggregation of edges between vertices in the two communities. 

\subsubsection{Two-Dimensional Graph Embedding}

Our partitioning based method needs a 2D embedding of vertices. To capture local connectivity and global community, we have three constraints for the resulting 2D graph embedding: 
\begin{enumerate}
  \item Connected vertices are embedded closely in the 2D latent space;  
   % such that their rectangles can be placed adjacent by our partitioning based layout method. 
  \item Vertices of the same community are close in the 2D space; 
  \item Different vertices cannot share the same latent vector to avoid all vertices degenerate into the same point in the latent space. 
\end{enumerate}
To obtain the 2D embedding based on the three constraints, we use force-directed layout for small graphs and project the resulting high-dimensional embedding to 2D space for large graphs. 

\textbf{Small graph. }When graph is small, many graph drawing methods are available. We select the force-directed layout method \cite{fruchterman1991graph} since it can effectively place connected vertices closely and form clusters naturally by using the metaphor of spring. For large graphs, force-directed layout methods may not perform well \cite{kobourov2012spring}. 
 % because the objective function usually has many local minima. }


\textbf{Large graph. } We map the resulting high-dimensional embedding of graphs into a 2D space. It is shown that node2vec has good performance on embedding large graphs in a high-dimensional space \cite{grover2016node2vec}. Hence, next, we aim to preserve the high-dimensional structures of vertices in the 2D space. To perform the multi-dimensional projection, in our paper, we require to preserve local proximities between vertex vectors as well as global communities of vertices. Various dimensionality reduction techniques can be used, in which \textit{t-SNE} \cite{maaten2008visualizing} shows its superiority on the capture of both local (i.e., proximity) and global (i.e., cluster) structures of multi-dimensional data. Hence, we select t-SNE to project the vectors of vertices from the high-dimensional latent space to a 2D latent space. 

The 2D embedding of graphs (e.g., Fig.~\ref{fig:les-miserables-subdividing} (a$_1$) and (b$_1$)) is used as a base of subsequent rectangular partitioning for graphs. After obtaining the 2D vectors of the vertices, the 2D latent vector of each community is equal to the average of the 2D vectors of vertices in the community. 


==> old_rgmap.tex <==

% %% bare_jrnl_compsoc.tex
% %% V1.4b
% %% 2015/08/26
% %% by Michael Shell
% %% See:
% %% http://www.michaelshell.org/
% %% for current contact information.
% %%
% %% This is a skeleton file demonstrating the use of IEEEtran.cls
% %% (requires IEEEtran.cls version 1.8b or later) with an IEEE
% %% Computer Society journal paper.
% %%
% %% Support sites:
% %% http://www.michaelshell.org/tex/ieeetran/
% %% http://www.ctan.org/pkg/ieeetran
% %% and
% %% http://www.ieee.org/

% %%*************************************************************************
% %% Legal Notice:
% %% This code is offered as-is without any warranty either expressed or
% %% implied; without even the implied warranty of MERCHANTABILITY or
% %% FITNESS FOR A PARTICULAR PURPOSE! 
% %% User assumes all risk.
% %% In no event shall the IEEE or any contributor to this code be liable for
% %% any damages or losses, including, but not limited to, incidental,
% %% consequential, or any other damages, resulting from the use or misuse
% %% of any information contained here.
% %%
% %% All comments are the opinions of their respective authors and are not
% %% necessarily endorsed by the IEEE.
% %%
% %% This work is distributed under the LaTeX Project Public License (LPPL)
% %% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
% %% distributed and modified. A copy of the LPPL, version 1.3, is included
% %% in the base LaTeX documentation of all distributions of LaTeX released
% %% 2003/12/01 or later.
% %% Retain all contribution notices and credits.
% %% ** Modified files should be clearly indicated as such, including  **
% %% ** renaming them and changing author support contact information. **
% %%*************************************************************************


% % *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% % *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% % *** with production work. The IEEE's font choices and paper sizes can   ***
% % *** trigger bugs that do not appear when using other class files.       ***                          ***
% % The testflow support page is at:
% % http://www.michaelshell.org/tex/testflow/


% \documentclass[10pt,journal,compsoc]{IEEEtran}
% %
% % If IEEEtran.cls has not been installed into the LaTeX system files,
% % manually specify the path to it like:
% % \documentclass[10pt,journal,compsoc]{../sty/IEEEtran}





% % Some very useful LaTeX packages include:
% % (uncomment the ones you want to load)


% % *** MISC UTILITY PACKAGES ***
% %
% %\usepackage{ifpdf}
% % Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% % compilation based on whether the output is pdf or dvi.
% % usage:
% % \ifpdf
% %   % pdf code
% % \else
% %   % dvi code
% % \fi
% % The latest version of ifpdf.sty can be obtained from:
% % http://www.ctan.org/pkg/ifpdf
% % Also, note that IEEEtran.cls V1.7 and later provides a builtin
% % \ifCLASSINFOpdf conditional that works the same way.
% % When switching from latex to pdflatex and vice-versa, the compiler may
% % have to be run twice to clear warning/error messages.






% % *** CITATION PACKAGES ***
% %
% \ifCLASSOPTIONcompsoc
%   % IEEE Computer Society needs nocompress option
%   % requires cite.sty v4.0 or later (November 2003)
%   \usepackage[nocompress]{cite}
% \else
%   % normal IEEE
%   \usepackage{cite}
% \fi
% % cite.sty was written by Donald Arseneau
% % V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% % \cite{} output to follow that of the IEEE. Loading the cite package will
% % result in citation numbers being automatically sorted and properly
% % "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% % cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% % \cite will automatically add leading space, if needed. Use cite.sty's
% % noadjust option (cite.sty V3.8 and later) if you want to turn this off
% % such as if a citation ever needs to be enclosed in parenthesis.
% % cite.sty is already installed on most LaTeX systems. Be sure and use
% % version 5.0 (2009-03-20) and later if using hyperref.sty.
% % The latest version can be obtained at:
% % http://www.ctan.org/pkg/cite
% % The documentation is contained in the cite.sty file itself.
% %
% % Note that some packages require special options to format as the Computer
% % Society requires. In particular, Computer Society  papers do not use
% % compressed citation ranges as is done in typical IEEE papers
% % (e.g., [1]-[4]). Instead, they list every citation separately in order
% % (e.g., [1], [2], [3], [4]). To get the latter we need to load the cite
% % package with the nocompress option which is supported by cite.sty v4.0
% % and later. Note also the use of a CLASSOPTION conditional provided by
% % IEEEtran.cls V1.7 and later.





% % *** GRAPHICS RELATED PACKAGES ***
% %
% \ifCLASSINFOpdf
%   \usepackage[pdftex]{graphicx}
%   % declare the path(s) where your graphic files are
%   \graphicspath{{figures/}{pictures/}{images/}{./}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
% \else
%   % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%   % will default to the driver specified in the system graphics.cfg if no
%   % driver is specified.
%   \usepackage[dvips]{graphicx}
%   % declare the path(s) where your graphic files are
%   \graphicspath{{../eps/}}
%   % and their extensions so you won't have to specify these with
%   % every instance of \includegraphics
%   \DeclareGraphicsExtensions{.eps}
% \fi
% % graphicx was written by David Carlisle and Sebastian Rahtz. It is
% % required if you want graphics, photos, etc. graphicx.sty is already
% % installed on most LaTeX systems. The latest version and documentation
% % can be obtained at: 
% % http://www.ctan.org/pkg/graphicx
% % Another good source of documentation is "Using Imported Graphics in
% % LaTeX2e" by Keith Reckdahl which can be found at:
% % http://www.ctan.org/pkg/epslatex
% %
% % latex, and pdflatex in dvi mode, support graphics in encapsulated
% % postscript (.eps) format. pdflatex in pdf mode supports graphics
% % in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% % that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% % not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% % which can result in "jaggedy"/blurry rendering of lines and letters as
% % well as large increases in file sizes.
% %
% % You can find documentation about the pdfTeX application at:
% % http://www.tug.org/applications/pdftex






% % *** MATH PACKAGES ***
% %
% \usepackage{amsmath}
% % A popular package from the American Mathematical Society that provides
% % many useful and powerful commands for dealing with mathematics.
% %
% % Note that the amsmath package sets \interdisplaylinepenalty to 10000
% % thus preventing page breaks from occurring within multiline equations. Use:
% %\interdisplaylinepenalty=2500
% % after loading amsmath to restore such page breaks as IEEEtran.cls normally
% % does. amsmath.sty is already installed on most LaTeX systems. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/amsmath





% % *** SPECIALIZED LIST PACKAGES ***
% %
% %\usepackage{algorithmic}
% % algorithmic.sty was written by Peter Williams and Rogerio Brito.
% % This package provides an algorithmic environment fo describing algorithms.
% % You can use the algorithmic environment in-text or within a figure
% % environment to provide for a floating algorithm. Do NOT use the algorithm
% % floating environment provided by algorithm.sty (by the same authors) or
% % algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% % algorithm float types and packages that provide these will not provide
% % correct IEEE style captions. The latest version and documentation of
% % algorithmic.sty can be obtained at:
% % http://www.ctan.org/pkg/algorithms
% % Also of interest may be the (relatively newer and more customizable)
% % algorithmicx.sty package by Szasz Janos:
% % http://www.ctan.org/pkg/algorithmicx




% % *** ALIGNMENT PACKAGES ***
% %
% %\usepackage{array}
% % Frank Mittelbach's and David Carlisle's array.sty patches and improves
% % the standard LaTeX2e array and tabular environments to provide better
% % appearance and additional user controls. As the default LaTeX2e table
% % generation code is lacking to the point of almost being broken with
% % respect to the quality of the end results, all users are strongly
% % advised to use an enhanced (at the very least that provided by array.sty)
% % set of table tools. array.sty is already installed on most systems. The
% % latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/array


% % IEEEtran contains the IEEEeqnarray family of commands that can be used to
% % generate multiline equations as well as matrices, tables, etc., of high
% % quality.




% % *** SUBFIGURE PACKAGES ***
% %\ifCLASSOPTIONcompsoc
% %  \usepackage[caption=false,font=footnotesize,labelfont=sf,textfont=sf]{subfig}
% %\else
% %  \usepackage[caption=false,font=footnotesize]{subfig}
% %\fi
% % subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% % for subfigure.sty, the latter of which is no longer maintained and is
% % incompatible with some LaTeX packages including fixltx2e. However,
% % subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% % which will override IEEEtran.cls' handling of captions and this will result
% % in non-IEEE style figure/table captions. To prevent this problem, be sure
% % and invoke subfig.sty's "caption=false" package option (available since
% % subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% % handling of captions.
% % Note that the Computer Society format requires a sans serif font rather
% % than the serif font used in traditional IEEE formatting and thus the need
% % to invoke different subfig.sty package options depending on whether
% % compsoc mode has been enabled.
% %
% % The latest version and documentation of subfig.sty can be obtained at:
% % http://www.ctan.org/pkg/subfig




% % *** FLOAT PACKAGES ***
% %
% %\usepackage{fixltx2e}
% % fixltx2e, the successor to the earlier fix2col.sty, was written by
% % Frank Mittelbach and David Carlisle. This package corrects a few problems
% % in the LaTeX2e kernel, the most notable of which is that in current
% % LaTeX2e releases, the ordering of single and double column floats is not
% % guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% % single column figure to be placed prior to an earlier double column
% % figure.
% % Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% % corrections already built into the system in which case a warning will
% % be issued if an attempt is made to load fixltx2e.sty as it is no longer
% % needed.
% % The latest version and documentation can be found at:
% % http://www.ctan.org/pkg/fixltx2e


% %\usepackage{stfloats}
% % stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% % the ability to do double column floats at the bottom of the page as well
% % as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% % LaTeX2e). It also provides a command:
% %\fnbelowfloat
% % to enable the placement of footnotes below bottom floats (the standard
% % LaTeX2e kernel puts them above bottom floats). This is an invasive package
% % which rewrites many portions of the LaTeX2e float routines. It may not work
% % with other packages that modify the LaTeX2e float routines. The latest
% % version and documentation can be obtained at:
% % http://www.ctan.org/pkg/stfloats
% % Do not use the stfloats baselinefloat ability as the IEEE does not allow
% % \baselineskip to stretch. Authors submitting work to the IEEE should note
% % that the IEEE rarely uses double column equations and that authors should try
% % to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% % packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% % such ways.
% % Do not attempt to use stfloats with fixltx2e as they are incompatible.
% % Instead, use Morten Hogholm'a dblfloatfix which combines the features
% % of both fixltx2e and stfloats:
% %
% % \usepackage{dblfloatfix}
% % The latest version can be found at:
% % http://www.ctan.org/pkg/dblfloatfix




% %\ifCLASSOPTIONcaptionsoff
% %  \usepackage[nomarkers]{endfloat}
% % \let\MYoriglatexcaption\caption
% % \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
% %\fi
% % endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% % Axel Sommerfeldt. This package may be useful when used in conjunction with 
% % IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% % submissions have lists of figures/tables at the end of the paper and that
% % figures/tables without any captions are placed on a page by themselves at
% % the end of the document. If needed, the draftcls IEEEtran class option or
% % \CLASSINPUTbaselinestretch interface can be used to increase the line
% % spacing as well. Be sure and use the nomarkers option of endfloat to
% % prevent endfloat from "marking" where the figures would have been placed
% % in the text. The two hack lines of code above are a slight modification of
% % that suggested by in the endfloat docs (section 8.4.1) to ensure that
% % the full captions always appear in the list of figures/tables - even if
% % the user used the short optional argument of \caption[]{}.
% % IEEE papers do not typically make use of \caption[]'s optional argument,
% % so this should not be an issue. A similar trick can be used to disable
% % captions of packages such as subfig.sty that lack options to turn off
% % the subcaptions:
% % For subfig.sty:
% % \let\MYorigsubfloat\subfloat
% % \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% % However, the above trick will not work if both optional arguments of
% % the \subfloat command are used. Furthermore, there needs to be a
% % description of each subfigure *somewhere* and endfloat does not add
% % subfigure captions to its list of figures. Thus, the best approach is to
% % avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% % and instead reference/explain all the subfigures within the main caption.
% % The latest version of endfloat.sty and its documentation can obtained at:
% % http://www.ctan.org/pkg/endfloat
% %
% % The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% % later in the document, say, to conditionally put the References on a 
% % page by themselves.




% % *** PDF, URL AND HYPERLINK PACKAGES ***
% %
% %\usepackage{url}
% % url.sty was written by Donald Arseneau. It provides better support for
% % handling and breaking URLs. url.sty is already installed on most LaTeX
% % systems. The latest version and documentation can be obtained at:
% % http://www.ctan.org/pkg/url
% % Basically, \url{my_url_here}.

% \usepackage{multirow} % for multirow of a table

% \usepackage{amsthm}
% \usepackage{commath}                  % for absolute and norm
% \usepackage{bm} % for bold math

% \usepackage{enumitem} % for styles of listed items like itemize, description

% \usepackage{caption}
% \usepackage{subcaption}

% \usepackage{breqn} % Automatic line breaking of displayed equations, math.

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}
% \theoremstyle{remark}
% \newtheorem*{remark}{Remark}


% \usepackage{xcolor} % use colors in Latex
% \usepackage[normalem]{ulem}
% % use blue color in the review stage
% \newcommand{\revision}[1]{\textcolor{blue}{#1}}
% % \newcommand{\remark}[1]{\textcolor{red}{#1}}
% %\newcommand\reduline{\bgroup\markoverwith{\textcolor{red}{\rule[0.5ex]{2pt}{0.4pt}}}\ULon}
% %\newcommand{\removed}[1]{\reduline{#1}}
% \newcommand{\removed}[1]{\textcolor{red}{\sout{#1}}}

% % \def \cleanversion{} % remove this comment to generate a clean version
% \ifx\cleanversion\undefined
% \else
%   \renewcommand{\revision}{}
%   % \renewcommand{\remark}{}
%   \renewcommand{\removed}[1]{\iffalse#1\fi}
% \fi

% \newcommand{\vect}[1]{\boldsymbol{#1}} %bold italic vector


% % *** Do not adjust lengths that control margins, column widths, etc. ***
% % *** Do not use packages that alter fonts (such as pslatex).         ***
% % There should be no need to do such things with IEEEtran.cls V1.6 and later.
% % (Unless specifically asked to do so by the journal or conference you plan
% % to submit to, of course. )


% % correct bad hyphenation here
% \hyphenation{op-tical net-works semi-conduc-tor}


% \begin{document}
% %
% % paper title
% % Titles are generally capitalized except for words such as a, an, and, as,
% % at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% % not capitalized unless they are the first or last word of the title.
% % Linebreaks \\ can be used within to get better formatting as desired.
% % Do not put math or special symbols in the title.
% \title{VMap: An Interactive Rectangular Space-filling Visualization for Vertex-centric Graph Exploration}
% % 
% %
% %
% % author names and IEEE memberships
% % note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% % a structure at a ~ so this keeps an author's name from being broken across
% % two lines.
% % use \thanks{} to gain access to the first footnote area
% % a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% % was not built to handle multiple paragraphs
% %
% %
% %\IEEEcompsocitemizethanks is a special \thanks that produces the bulleted
% % lists the Computer Society journals use for "first footnote" author
% % affiliations. Use \IEEEcompsocthanksitem which works much like \item
% % for each affiliation group. When not in compsoc mode,
% % \IEEEcompsocitemizethanks becomes like \thanks and
% % \IEEEcompsocthanksitem becomes a line break with idention. This
% % facilitates dual compilation, although admittedly the differences in the
% % desired content of \author between the different types of papers makes a
% % one-size-fits-all approach a daunting prospect. For instance, compsoc 
% % journal papers have the author affiliations above the "Manuscript
% % received ..."  text while in non-compsoc journals this is reversed. Sigh.


% \author{Jiayi~Xu
%         and~Han-Wei~Shen
%         % ,~\IEEEmembership{Member,~IEEE}%
%         % John~Doe,~\IEEEmembership{Fellow,~OSA,}
%         % and~Jane~Doe,~\IEEEmembership{Life~Fellow,~IEEE}% <-this % stops a space
% \IEEEcompsocitemizethanks{\IEEEcompsocthanksitem J. Xu is with the Department of Computer Science and Engineering, The Ohio State University, Columbus, OH, 43210.\protect\\
% % note need leading \protect in front of \\ to get a newline within \thanks as
% % \\ is fragile and will error, could use \hfil\break instead.
% E-mail: xu.2205@osu.edu
% \IEEEcompsocthanksitem H.-W. Shen is with the Department of Computer Science and Engineering, The Ohio State University, Columbus, OH, 43210.\protect\\
% E-mail: shen.94@osu.edu}% <-this % stops an unwanted space
% \thanks{Manuscript received April 19, 2005; revised August 26, 2015.}}


% % \author{Michael~Shell,~\IEEEmembership{Member,~IEEE,}
% %         John~Doe,~\IEEEmembership{Fellow,~OSA,}
% %         and~Jane~Doe,~\IEEEmembership{Life~Fellow,~IEEE}% <-this % stops a space
% % \IEEEcompsocitemizethanks{\IEEEcompsocthanksitem M. Shell was with the Department
% % of Electrical and Computer Engineering, Georgia Institute of Technology, Atlanta,
% % GA, 30332.\protect\\
% % % note need leading \protect in front of \\ to get a newline within \thanks as
% % % \\ is fragile and will error, could use \hfil\break instead.
% % E-mail: see http://www.michaelshell.org/contact.html
% % \IEEEcompsocthanksitem J. Doe and J. Doe are with Anonymous University.}% <-this % stops an unwanted space
% % \thanks{Manuscript received April 19, 2005; revised August 26, 2015.}}

% % note the % following the last \IEEEmembership and also \thanks - 
% % these prevent an unwanted space from occurring between the last author name
% % and the end of the author line. i.e., if you had this:
% % 
% % \author{....lastname \thanks{...} \thanks{...} }
% %                     ^------------^------------^----Do not want these spaces!
% %
% % a space would be appended to the last name and could cause every name on that
% % line to be shifted left slightly. This is one of those "LaTeX things". For
% % instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% % "AB" then you have to do: "\textbf{A}\textbf{B}"
% % \thanks is no different in this regard, so shield the last } of each \thanks
% % that ends a line with a % and do not let a space in before the next \thanks.
% % Spaces after \IEEEmembership other than the last one are OK (and needed) as
% % you are supposed to have spaces between the names. For what it is worth,
% % this is a minor point as most people would not even notice if the said evil
% % space somehow managed to creep in.



% % The paper headers
% \markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
% {Xu \MakeLowercase{\textit{et al.}}: VMap: a \textbf{R}ectangular Space-filling Visualization for Vertex-Weighted \textbf{G}raph}
% % The only time the second header will appear is for the odd numbered pages
% % after the title page when using the twoside option.
% % 
% % *** Note that you probably will NOT want to include the author's ***
% % *** name in the headers of peer review papers.                   ***
% % You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% % you desire.



% % The publisher's ID mark at the bottom of the page is less important with
% % Computer Society journal papers as those publications place the marks
% % outside of the main text columns and, therefore, unlike regular IEEE
% % journals, the available text space is not reduced by their presence.
% % If you want to put a publisher's ID mark on the page you can do it like
% % this:
% %\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% % or like this to get the Computer Society new two part style.
% %\IEEEpubid{\makebox[\columnwidth]{\hfill 0000--0000/00/\$00.00~\copyright~2015 IEEE}%
% %\hspace{\columnsep}\makebox[\columnwidth]{Published by the IEEE Computer Society\hfill}}
% % Remember, if you use this you must call \IEEEpubidadjcol in the second
% % column for its text to clear the IEEEpubid mark (Computer Society jorunal
% % papers don't need this extra clearance.)



% % use for special paper notices
% %\IEEEspecialpapernotice{(Invited Paper)}



% % for Computer Society papers, we must declare the abstract and index terms
% % PRIOR to the title within the \IEEEtitleabstractindextext IEEEtran
% % command as these need to go into the title area created by \maketitle.
% % As a general rule, do not put math, special symbols or citations
% % in the abstract or keywords.
% \IEEEtitleabstractindextext{%
% \begin{abstract}
% \revision{
% % Space-filling maps utilize the screen space as much as possible and split it into subdivisions to represent data elements. Treemaps, among these approaches, are well-known for visualizing hierarchical vertex-weighted trees by using nesting and compact rectangles. As a general form of vertex-weighted tree, vertex-weighted graphs refer to graphs with numeric attributes attached on vertices, and are common in real-world applications such as social networks and cartograms. However, rectangular space-filling designs for vertex-weighted graphs are little studied. There are two challenges for this problem. The first is how to place graph edges with minimal vertex-edge occlusion. The second is how to produce and arrange rectangles of vertices by considering multiple factors including weights of vertices, adjacency of vertices, and aspect ratios of rectangles. In this paper, we propose VMap to tackle the problem and explore graphs in a vertex-centric way. VMap is similar to a treemap visually;
% % differently, graph edges are embedded between rectangles. To route edges, we propose a two-stage adjustment approach for rectangular layout to insert a border space between rectangles, which avoids vertex-edge intersection. To produce rectangular layout of graph vertices, we first embed graphs into two-dimensional (2D) space. Then, we propose a Desired-Aspect-Ratio (DAR) partitioning algorithm to subdivide the 2D embedding of vertices into rectangles. The resulting rectangular layout has better aspect ratio quality on synthetic data by compared with the existing best method for the rectangular partitioning of 2D points. We further introduce the simulated annealing method for the arrangement of rectangles to support trade-offs amongst aspect ratio quality and the encoding accuracies of vertices' weights and adjacency. Our method can achieve better encoding accuracy, and get faster speed with three to four orders of magnitude on three real-world datasets by compared with existing methods for rectangular layout of graph vertices. Finally, we illustrate the effectiveness of VMap for vertex-centric graph exploration by three applications including visualizing social network, representing academic community, and displaying geographic information. 
% }
% \end{abstract}

% % Similar to a (rectangular) treemap, VMap represents each vertex by a rectangle and encode its weight by the area of the rectangle; when graphs have hierarchical structures, rectangles of low-level vertices are nested within high-level rectangles. 

% % Note that keywords are not normally used for peerreview papers.
% \begin{IEEEkeywords}
% Rectangular space-filling visualization, rectangular layout adjustment, graph layout. 
% \end{IEEEkeywords}}


% % make the title area
% \maketitle


% % To allow for easy dual compilation without having to reenter the
% % abstract/keywords data, the \IEEEtitleabstractindextext text will
% % not be used in maketitle, but will appear (i.e., to be "transported")
% % here as \IEEEdisplaynontitleabstractindextext when the compsoc 
% % or transmag modes are not selected <OR> if conference mode is selected 
% % - because all conference papers position the abstract like regular
% % papers do.
% \IEEEdisplaynontitleabstractindextext
% % \IEEEdisplaynontitleabstractindextext has no effect when using
% % compsoc or transmag under a non-conference mode.



% % For peer review papers, you can put extra information on the cover
% % page as needed:
% % \ifCLASSOPTIONpeerreview
% % \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% % \fi
% %
% % For peerreview papers, this IEEEtran command inserts a page break and
% % creates the second title. It will be ignored for other modes.
% \IEEEpeerreviewmaketitle



% \IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
% % Computer Society journal (but not conference!) papers do something unusual
% % with the very first section heading (almost always called "Introduction").
% % They place it ABOVE the main text! IEEEtran.cls does not automatically do
% % this for you, but you can achieve this effect with the provided
% % \IEEEraisesectionheading{} command. Note the need to keep any \label that
% % is to refer to the section immediately after \section in the above as
% % \IEEEraisesectionheading puts \section within a raised box.




% % The very first letter is a 2 line initial drop letter followed
% % by the rest of the first word in caps (small caps for compsoc).
% % 
% % form to use if the first word consists of a single letter:
% % \IEEEPARstart{A}{demo} file is ....
% % 
% % form to use if you need the single drop letter followed by
% % normal text (unknown if ever used by the IEEE):
% % \IEEEPARstart{A}{}demo file is ....
% % 
% % Some journals put the first two words in caps:
% % \IEEEPARstart{T}{his demo} file is ....
% % 
% % Here we have the typical use of a "T" for an initial drop letter
% % and "HIS" in caps to complete the first word.

% \input{1_introduction}

% \section{Related Works}
% \input{2_related_works}

% \section{Preliminary and Design Requirements} \label{sect:requirements}
% \input{3_requirements}



% \section{Overview of VMap}

% We provide the framework overview of VMap to satisfy aforementioned requirements. We embed a given vertex-weighted graph into a high-dimensional latent space. The resulting latent vectors of vertices are used for the clustering of vertices to estimate communities (Requirement 2-1). Also, we acquire 2D embedding of vertices by either using force-directed layout for small graphs or projecting the high-dimensional latent vectors to 2D space for large graphs. The partitioning based rectangular layout method for vertices can ensure the property of space filling (Requirement 1-3). We arrange rectangles for clusters of vertices first, and arrange vertices within rectangles of clusters second (Requirement 2-1). When rectangles are being arranged, the aspect ratio of each rectangle is targeted at a desired number (1.5 by default) (Requirement 1-4), and zero areal error is guaranteed (Requirement 1-1). Through trade-off against areal error and aspect ratio loss, we optimize connected vertices to be adjacent by using simulated annealing hence the connections between vertices can be represented by contacts between rectangles as many as possible (Requirement 1-2). However, when edges become dense, it becomes impossible to preserve all edges through the contacts between rectangles. In our paper, we further open a border space between rectangles to route edges amongst vertices (Requirement 1-2), and users can identify more edges between vertices through interactions (Requirement 2-2). Since the requirement of low areal error (Requirement 1-1), a two-stage rectangle adjustment technique is devised carefully without introducing additional areal distortion. Visual elements for edges of vertices are placed inside the border space. Then, we can link adjacent rectangles and support queries of paths of vertices which are far away (Requirement 2-2). We give specific solutions for each module of the framework hereafter. 

% % % \setlength{\belowcaptionskip}{-10pt}
% % \begin{figure*}[htb]
% % \centering
% % \captionsetup[subfigure]{} %{labelformat=empty}
 
 
% %  % \bigskip
 
% %   % \vspace{-1em}
% %   \caption{ }
% %   \label{fig:les-miserables-graph}
% % \end{figure*}
% % % \setlength{\belowcaptionskip}{0pt}

% % \setlength{\belowcaptionskip}{-10pt}



% \begin{figure*}[tb]
% \centering
% \captionsetup[subfigure]{labelformat=empty}

% \begin{subfigure}[b]{0.3\linewidth}
%  \includegraphics[width=\columnwidth]{les-miserables-graph-force}
%  \caption{(a$_1$)}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.3\linewidth}
%    \includegraphics[width=\columnwidth]{partitioning/les-miserables-rgmap-plus-graph}
%    \caption{(a$_2$)}
%  \end{subfigure}
%  \hfill
%  \begin{subfigure}[b]{0.3\linewidth}
%    \includegraphics[width=\columnwidth]{partitioning/les-miserables-rgmap}
%    \caption{(a$_3$)}
%  \end{subfigure}

% \bigskip

% \begin{subfigure}[b]{0.3\linewidth}
%  \includegraphics[width=\columnwidth]{les-miserables-graph}
%  \caption{(b$_2$)}
% \end{subfigure} 
% \hfill
%  \begin{subfigure}[b]{0.3\linewidth}
%    \includegraphics[width=\columnwidth]{partitioning/les-miserables-rgmap-plus-graph-node2vec}
%    \caption{(b$_2$)}
%  \end{subfigure} 
%  \hfill
%  \begin{subfigure}[b]{0.3\linewidth}
%    \includegraphics[width=\columnwidth]{partitioning/les-miserables-rgmap-node2vec}
%    \caption{(b$_3$)}
%  \end{subfigure} 

% % \bigskip
 
%   % \vspace{-1em}
%   \caption{\revision{We show a vertex-weighted graph for characters in a novel \textit{Les Mis\'{e}rables} \cite{hugo1887miserables}, which is illustrated in Sect.~\ref{sect:app_les} with details. (a$_1$) The 2D graph embedding is produced by a graph drawing method, force-directed layout \cite{fruchterman1991graph}. (b$_1$) The 2D graph embedding is produced by a combined method of node2vec and t-SNE. Both methods preserve local connectivity and global clusters well. Each vertex is represented by a circle, and its weight is encoded by the radius of circle. Related vertices are connected by links. Colors encode clusters of vertices, and are suggested by ColorBrewer \cite{brewer2019colorbrewer}. By using the partitioning based DAR heuristic method, we show the second column for the rectangular subdivisions of the network. 
%   % The positions of vertices on the node-link diagrams are set to the centers of their corresponding rectangles. 
%   We only show the partitioned rectangles on the third column. Thickness of frame lines encodes the sequential order of the partitioning; thicker cuts occur earlier by using the DAR algorithm. }
%   % Also, we draw the node-link diagrams solely on (c) and (f). 
%   }
%   \label{fig:les-miserables-subdividing}
% \end{figure*}
% % \setlength{\belowcaptionskip}{0pt}



% \section{Rectangular Space-filling Subdivision for Graph Vertices}
% This section describes how to produce rectangular subdivisions for graph vertices. We first extract clusters of vertices based on high-dimensional embedding of graphs. We next subdivide vertices rectangularly by using a two-dimensional embedding of graphs and performing a desired-aspect-ratio rectangular subdivision on the resulting 2D embedding space. Moreover, we apply the simulated annealing approach to optimize the total of areal error, topological error, and aspect ratio loss for the resulting subdivisions. 

% \subsection{Graph Embedding}
% \input{5_graph_embedding}

% \subsection{Desired-Aspect-Ratio (DAR) Heuristic Partitioning Algorithm}
% \input{6_layout_methods}


% \section{Border Encoding for Graph Edges}
% \input{7_borders}



% \section{Applications for Vertex-centric Exploration of Graphs}
% \input{8_applications}

% % \section{Discussions}


% % \subsection{Graphs with Different Topological Structures}


% % Limitations: Not good for dense graphs such as complete graph

% % Spanning tree based algorithm
%   % We can exhaust all possi... test by starting the arrangement with every vertex as the root, and select the one with the best quality among all the results; however, it is time-consuming. 


% % Note that since the partitionin of treemap \cite{johnson1991tree} can also be stored by a kd-tree; hence, our two-stage adjument is also available for treemaps to remove the areal distortion by borders and labels. 

% % If someone is eager to acquire an equal-width of borders, we can perform a top-down adjustment again but note that the second iteration of the top-down adjustment don't need to consider the area of junctions. In addition, iteratively performing the top-down and bottom-up adjustments can reduce the error of borders further? 


% % Limitation, we do not minimize the topological error. Mention the definition of topological error, say we can incorporate the error when we place rectangles in the spanning tree based method. 


% % \subsection{Discussion for Two Layout Variants on Perservation of Graph Edges}

% % and (3) the topological losses
% % The \textit{topological loss} is measured by the number of edges that are lost divided by total number of edges on the raw graph. 
% % the topological loss for the partitioning based method is $68.11\%$, and for spanning tree based method is $58.27\%$.





% % \subsection{Qualitative Discussion}


% % Partitioning based methods have few limits. 
% % If the graph is not connected, the spanning tree based method relys on the partitioning based method. 

% % The given tree structure is explicitly preserved by the spanning tree based method. Hence, spanning Tree based method is proper for tree-like inputs, and can control some edges, for example, to give some edges high weights such the edges can be preserved in the spanning tree and be preserved by the contacts between rectangles. 


% % If no tree of the given graph is requried to be preserved, we introduce a more straightforward partitioning based method below. 

% % Partitioning based methods can place the vertices with high centrality of the same cluster at the center of the cluster. 

% % Moreover, the rectangular results of partitioning based methods DO NOT satisfy the \textit{area-universal} property. 
%   %  Since when expanding some vertices, the adjacecy will change!!!! 

% % Eppstein et al. \cite{eppstein2012area} described ``a layout is area-universal if any assignment of areas to rectangles can be realized by a combinatorially equivalent rectangular layout''; two rectangular layouts are combinatorially equivalent means that the rectangles on the two layouts are order-equivalent in the plane \cite{eppstein2012area}. The area-universal property is important for graphs with time-varying weights or vertices having multiple weights; for these cases, we desire the arrangement of rectangles to have a stable 2D ordering in each visualization. 

% % Technically speaking, we can use the same resulting partitioning structure stored in the k-d tree for different weights of vertices; we only need to re-compute widths and heights of subdividing rectangles by traversing the k-d tree. 


% \section{Discussions}

% We discuss benefits and limitations of VMap from different perspectives in the following. 

% \revision{
% \textbf{Values of VMap. }VMap is useful for graph visualization from five aspects. 
% First, since VMap layout is based on graph embedding, the advantages of graph embedding are inherited such as the ability to capture global communities (e.g., Fig.~\ref{fig:teaser}) and to place connected entities closely (e.g., Fig.~\ref{fig:vis_pub_case}b). Also, since the neighborhood and adjacency of provinces of Netherlands are well preserved in Fig.~\ref{fig:netherlands} by VMap, VMap is a good choice on presenting geographic information. 
% Second, due to the space-filling nature, VMap has higher space-usage efficiency of the screen by compared with node-link diagram (e.g., Fig.~\ref{fig:les-miserables-subdividing}) and cartogram (e.g., Fig.~\ref{fig:netherlands}). 
% Third, because we route edges between rectangles, the visual clutter and vertex-edge intersection are reduced by comparing with overlying links on rectangles (e.g., \cite{fekete2003interactive}). 
% To display information of vertices, fourth, because VMap offers a rectangle for each vertex, labels of vertices such as names of persons (\textit{Les Mis\'{e}rables} Data and VIS publication data) and names of provinces (Netherlands data) can be organized regularly and shown clearly. 
% Fifth, with respect to the perceptual judgement of vertices' values, Kong et al. \cite{kong2010perceptual} showed that space-filling rectangular visualizations (e.g., treemaps \cite{Shneiderman1992, johnson1991tree}) have higher accuracies than bar charts when the number of vertices is large, since the space-filling property leads to an efficient space usage. 
% % When the number of vertices is small, although rectangular visualizations are not better than bar charts and pie charts from the studies \cite{kong2010perceptual, heer2010crowdsourcing}, it is hard to acquire graph structures from the bars and pies. 
% Moreover, the results of the study by Heer et al. \cite{heer2010crowdsourcing} show that the rectangular representations are better than circular ones on the average in terms of the proportional judgment. }

% \revision{
% \textbf{Preservation of topological structures. }
% Static VMap uses bridges between rectangles to show direct connections between adjacent rectangles, which is useful for sparse graphs (e.g., pink and purple clusters of Fig.~\ref{fig:les-miserables-rgmap-final}) or planar graphs (e.g., Fig.~\ref{fig:netherlands}). When the number of edges increases, topological structures with dense edges (e.g., complete graphs) cannot be represented well by static VMap, which is a main limitation of the static VMap due to the limited adjacencies of rectangles. To remedy the limitation, 
% % when edges have weights, this static visualization can also be optimized to preserve edges with high weights (e.g., Fig.~\ref{fig:les-miserables-rgmap-final}d). Moreover, 
% by the help of interactions, VMap supports query for egocentric network of a selected rectangle and shorted-hop path between two selected rectangles. }

% \textbf{Trade-off topological error against areal error and aspect ratio loss. }
% Results on Table \ref{table:optimization_topology} indicate that our method can improve topological performance by increasing the weight of topological error, $\lambda_{t}$, while, with the sacrifice of areal encoding and aspect ratio quality, which brings flexibility when users require different performance for topological encoding, areal encoding, and aspect ratio on distinct applications. 


% \revision{
% \textbf{Distortion of border width. }
% After performing the fine bottom-up adjustment, a limitation is that the widths of some borders may be scaled so the widths of these borders have a small distortion and are not $d$ exactly. However, because only the low areal error is our design requirement in Sect.~\ref{sect:requirements}, the small distortion of some border widths is acceptable. }
% % After the coarse top-down adjustment, the areal error of the \textit{Les Mis\'{e}rables} data is $1.05 \times 10^{-4}$. The fine bottom-up adjustment reduce the areal error further to zero. 
% % theoretically ensures faithful areal encoding, and experimentally reduce the areal error of the coarse adjustment to $8.49 \times 10^{-18}$ due to the limit of arithmetic precision of numeric value.

% \revision{
% \textbf{Generation of treemap by using VMap. }
% Treemaps \cite{Shneiderman1992, johnson1991tree} are well-know for their ability to display hierarchical trees. Because tree is a special form of graph, we can use our method to produce treemaps as well. To produce treemaps by our method, we treat each hierarchical tree as one graph and embeds this graph into a 2D space either by using the force-directed layout or the combination of node2vec and t-SNE.  After we acquire 2D embedding of the hierarchical tree, we use our partitioning based method to generate rectangles for vertices on the hierarchical tree layer by layer which ensures rectangles of high-level vertices enclose low-level vertices. The limitation is that the quality of resulting treemaps is highly relevant to the 2D graph embedding of hierarchical trees. }


% \section{Conclusion}

% \revision{
% In this paper, we present a novel rectangular space-filling design called VMap to visualize vertex-weighted graphs. VMap is effective to display information attached on vertices including weights and labels. Also, VMap displays global communities of vertices in a compact way and places related individuals closely. The DAR partitioning method of VMap achieves lower aspect ratio loss of resulting rectangles than the equal-weight partitioning based method for synthetic 2D spatial data. Moreover, when introduced simulated annealing method to optimize the weighted loss of areal error, topological error, and aspect ratio loss, the layout method of VMap outperforms existing optimization based methods on total error and processing time of three real-world datasets. To route edges, the border space is inserted between rectangles, which prevents vertex-edge occlusion. Static VMap visualizes edges by rectangular bridges between rectangles and is optimized to preserve as many edges as possible. By interactions, VMap intuitively shows the egocentric network of a selected entity and displays shortest-hop path between a pair of selected individuals. Finally, VMap is applied on three visualization applications including social network, academic community, and cartogram effectively. 
% }


% % or to preserve edges with top-$k$ largest weights

% % To answer queries for specific topological structures locally? . 

% % Cycle/loop/star. Effectiveness of Graph Structure Perception? Hard to perserve. 

% % By comparing the node-link style, the rectangular representations of graphs are more proper for sparse graphs since the rectangular representations of dense graphs lose more connections. 

% % In the future, we will consider more constraints from the data for the rectangular representations. For example, 
% % + Subtrees have hierarchy? E.g., finger branches merge
% % + Spatial info? E.g., each node has a location
% % + Temporal info? E.g., each node has a timestamp

% % Use which network embedding methods?  
% %   Compare with other network embedding methods























% % if have a single appendix:
% %\appendix[Proof of the Zonklar Equations]
% % or
% %\appendix  % for no appendix heading
% % do not use \section anymore after \appendix, only \section*
% % is possibly needed

% % use appendices with more than one appendix
% % then use \section to start each appendix
% % you must declare a \section before using any
% % \subsection or using \label (\appendices by itself
% % starts a section numbered zero.)
% %


% % \appendices
% % \section{Proof of the First Zonklar Equation}
% % Appendix one text goes here.

% % % you can choose not to have a title for an appendix
% % % if you want by leaving the argument blank
% % \section{}
% % Appendix two text goes here.


% % % use section* for acknowledgment
% % \ifCLASSOPTIONcompsoc
% %   % The Computer Society usually uses the plural form
% %   \section*{Acknowledgments}
% % \else
% %   % regular IEEE prefers the singular form
% %   \section*{Acknowledgment}
% % \fi


% % The authors would like to thank...


% % Can use something like this to put references on a page
% % by themselves when using endfloat and the captionsoff option.
% \ifCLASSOPTIONcaptionsoff
%   \newpage
% \fi



% % trigger a \newpage just before the given reference
% % number - used to balance the columns on the last page
% % adjust value as needed - may need to be readjusted if
% % the document is modified later
% %\IEEEtriggeratref{8}
% % The "triggered" command can be changed if desired:
% %\IEEEtriggercmd{\enlargethispage{-5in}}

% % references section

% % can use a bibliography generated by BibTeX as a .bbl file
% % BibTeX documentation can be easily obtained at:
% % http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% % The IEEEtran BibTeX style support page is at:
% % http://www.michaelshell.org/tex/ieeetran/bibtex/
% \bibliographystyle{IEEEtran}
% % argument is your BibTeX string definitions and bibliography database(s)
% \bibliography{rgmap}
% %
% % <OR> manually copy in the resultant .bbl file
% % set second argument of \begin to the number of references
% % (used to reserve space for the reference number labels box)
% % \begin{thebibliography}{1}

% % \bibitem{IEEEhowto:kopka}
% % H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
% %   0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

% % \end{thebibliography}

% % biography section
% % 
% % If you have an EPS/PDF photo (graphicx package needed) extra braces are
% % needed around the contents of the optional argument to biography to prevent
% % the LaTeX parser from getting confused when it sees the complicated
% % \includegraphics command within an optional argument. (You could create
% % your own custom macro containing the \includegraphics command to make things
% % simpler here.)
% %\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% % or if you just want to reserve a space for a photo:

% % \begin{IEEEbiography}{Michael Shell}
% % Biography text here.
% % \end{IEEEbiography}

% % % if you will not have a photo at all:
% % \begin{IEEEbiographynophoto}{John Doe}
% % Biography text here.
% % \end{IEEEbiographynophoto}

% % % insert where needed to balance the two columns on the last page with
% % % biographies
% % %\newpage

% % \begin{IEEEbiographynophoto}{Jane Doe}
% % Biography text here.
% % \end{IEEEbiographynophoto}

% % You can push biographies down or up by placing
% % a \vfill before or after them. The appropriate
% % use of \vfill depends on what kind of text is
% % on the last page and whether or not the columns
% % are being equalized.

% %\vfill

% % Can be used to pull up biographies so that the bottom of the last one
% % is flush with the other column.
% %\enlargethispage{-5in}



% % that's all folks
% \end{document}



